Nonlocality under Computational Assumptions

Nonlocality and its connections to entanglement are fundamental features of quantum mechanics that have found numerous applications in quantum information science. A set of correlations is said to be nonlocal if it cannot be reproduced by spacelike-separated parties sharing randomness and performing local operations. An important practical consideration is that the runtime of the parties has to be shorter than the time it takes light to travel between them. One way to model this restriction is to assume that the parties are computationally bounded. We therefore initiate the study of nonlocality under computational assumptions and derive the following results: (a) We define the set $\mathsf{NeL}$ (not-efficiently-local) as consisting of all bipartite states whose correlations arising from local measurements cannot be reproduced with shared randomness and \emph{polynomial-time} local operations. (b) Under the assumption that the Learning With Errors problem cannot be solved in \emph{quantum} polynomial-time, we show that $\mathsf{NeL}=\mathsf{ENT}$, where $\mathsf{ENT}$ is the set of \emph{all} bipartite entangled states (pure and mixed). This is in contrast to the standard notion of nonlocality where it is known that some entangled states, e.g. Werner states, are local. In essence, we show that there exist (efficient) local measurements producing correlations that cannot be reproduced through shared randomness and quantum polynomial-time computation. (c) We prove that if $\mathsf{NeL}=\mathsf{ENT}$ unconditionally, then $\mathsf{BQP}\neq\mathsf{PP}$. In other words, the ability to certify all bipartite entangled states against computationally bounded adversaries gives a non-trivial separation of complexity classes. (d) Using (c), we show that a certain natural class of 1-round delegated quantum computation protocols that are sound against $\mathsf{PP}$ provers cannot exist.

==> oldintro.tex <==
\section{Old intro}

%These results imply that the relation between entanglement and nonlocality is more nuanced.

On the surface, these two types of advantages look very different but there's a growing body of work finding connections between the two notions.

The problem of factoring has a property that given the output of the algorithm it is easy for a classical algorithm to check that is is correct, i.e. factoring is in $\NP$.
However, it is believed that quantum polynomial time computers ($\BQP$) can solve problems outside of $\NP$.
%But even if a quantum computer solves a given problem faster than a classical one there remains a question of verification, i.e. how can a classical machine easily check that the problem was solved correctly?
This suggests considering the following problem.
In the delegation of quantum computation (DQC) we aim to design a protocol in which a classical client delegates and verifies the execution of a quantum circuit to a quantum prover(s).
DQC can be thought of as an efficiently verifiable quantum advantage.

DQC was considered in both, a single and multiprover setting.
In the single prover setting it was shown that the quantum hardness of LWE implies DQC assuming that the prover is in $\BQP$.
Firstly, many works considered DQC in a multiprover setting. 
These protocols are mostly based on the nonlocality of quantum states, some rigidity properties of EPR pairs more concretely.
Thus we can see it as using nonlocality for certifying quantum advantage.
A recent work \cite{advantagefromnonlocality} demonstrated how, using quantum fully holomorphic encryption, to design a single-prover quantum advantage experiment out of any non-local game.

We contribute to understanding these connections.


\subsection{Introduction}
Axioms of quantum theory define states of a quantum system to be operators on a Hilbert space. 
Consider a state $\rho_{AB}$ that is shared between two parties $\alice$ and $\bob$. 
Such a state can fall into one of the following categories. Either it is a \emph{separable state}, i.e., a state that can be written as $\sigma_{AB} =\sum_i p_i \sigma_A^{(i)} \otimes \sigma_B^{(i)}$. 
If not, it is called \emph{entangled}. 
This separation relies purely on a mathematical formalism. 
The question of Entanglement = Nonlocality ($\ENT \stackrel{?}{=} \NONL$) asks whether there is an operational distinction between separable and entangled states.

More formally we ask if it is true that for every entangled state $\rho_{AB}$ there exists a game between $\alice, \bob$ and a verifier $\ver$ that distinguishes between two cases: (i) $\alice$ and $\bob$ share $\rho_{AB}$ versus (ii) $\alice$ and $\bob$ share only a separable state $\sigma_{AB}$. 
The game is akin to the multi-prover interactive proof setup. 
More concretely, $\alice$ and $\bob$ are spatially separated so that they cannot communicate, then $\ver$ exchanges messages with both of them and, in the end, decides if $\alice$ and $\bob$ held only an entangled state. 
The verifier $\ver$ wins the game if her answer is correct with high probability. 
If such a game exists for a state $\rho_{AB}$ then we call $\rho_{AB}$ \textit{non-local}.
Whether every entangled state is non-local is the $\ENT \stackrel{?}{=} \NONL$ question.

The seminal paper \cite{bell} initiated the study of quantum nonlocality, i.e. of correlations obtained from performing local measurements on entangled states that do not have classical analogs. 
There, it was shown that there exists an entangled state (an EPR pair) for which there exist an experiment distinguishing cases (i) and (ii). 
This proved that classical and quantum theories give different predictions, or, in our language, that at least some entangled states are non-local.

Initially, it was believed that $\ENT = \NL$. 
This is in fact true for pure states (\cite{gisinpurestatesarenonlocal}). 
However, in 1989, Werner introduced (\cite{wernerprojective}) entangled states, for which a local model can be constructed. 
What this means is that all correlations obtainable with these entangled states can be reproduced in a setting where $\alice$ and $\bob$ hold only a separable state. 
The first simulation reproduced projective measurements only but it was later generalized to all POVMs (\cite{barrettmodel}). 
These results imply that no experiment can distinguish the two cases for these special entangled states, which in turn implies that the relation between $\ENT$ and $\NL$ is more nuanced.

The above simulations suggest that no operational notion exists behind the mathematical concept of entanglement, at least in this model. 
As a consequence new models were introduced and in some cases, equality was proven. 
One can tweak the model in many ways, e.g., allowing quantum communication between $\ver$ and $\alice,\bob$, considering multi-round games instead of a one-question, one-answer setting of the Bell scenario, or allowing more than one copy of $\rho_{AB}$ to be accessible at a time. 
It is probably fair to say that a satisfying answer to the $\ENT = \NL$ has not been found to date. 
For a more detailed history of the problem see Section~\ref{sec:history}.
